An Extension of hibi's palindromic theorem

Hibi showed that the polynomial in the numerator of the Ehrhart series of a reflexive polytope is palindromic. We proved that those in the numerator of the Ehrhart series of every graph polytope (defined later) of the bipartite graph is palindromic. From this, one of the conjectures (raised in the A205497 of OEIS \cite{[O]}) follows immediately.

==> 1310523.tex <==
%auto-ignore
